On the Minimum Distance of Non Binary LDPC Codes

Minimum distance is an important parameter of a linear error correcting code. For improved performance of binary Low Density Parity Check (LDPC) codes, we need to have the minimum distance grow fast with n, the codelength. However, the best we can hope for is a linear growth in dmin with n. For binary LDPC codes, the necessary and sufficient conditions on the LDPC ensemble parameters, to ensure linear growth of minimum distance is well established. In the case of non-binary LDPC codes, the structure of logarithmic weight codewords is different from that of binary codes. We have carried out a preliminary study on the logarithmic bound on the the minimum distance of non-binary LDPC code ensembles. In particular, we have investigated certain configurations which would lead to low weight codewords. A set of simulations are performed to identify some of these configurations. Finally, we have provided a bound on the logarithmic minimum distance of nonbinary codes, using a strategy similar to the girth bound for binary codes. This bound has the same asymptotic behaviour as that of binary codes.

==> pgflibraryarrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryarrows.code.tex,v 1.5 2006/10/11 15:22:26 tantau Exp $


% A square bracket shaped arrow

\pgfarrowsdeclare{[}{]}
{
  \@tempdima=1pt%
  \advance\@tempdima by1.25\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdima}
  \pgfarrowsrightextend{.5\pgflinewidth}
}
{
  \@tempdima=2pt%
  \advance\@tempdima by1.5\pgflinewidth%
  \@tempdimb=\@tempdima%
  \advance\@tempdimb by\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfpoint{-.5\@tempdimb}{-\@tempdima}}
  \pgfpathlineto{\pgfpoint{0pt}{-\@tempdima}}
  \pgfpathlineto{\pgfpoint{0pt}{\@tempdima}}
  \pgfpathlineto{\pgfpoint{-.5\@tempdimb}{\@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{]}{[}{[}{]}


% A round bracket shaped arrow

\pgfarrowsdeclare{(}{)}
{
  \@tempdima=2pt%
  \advance\@tempdima by1.5\pgflinewidth%
  \@tempdimb=0.0625\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
  \@tempdimb=0.5\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
}
{
  \@tempdima=2pt%
  \advance\@tempdima by1.5\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpoint{-.5\@tempdima}{-\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{.25\@tempdima}{-.5\@tempdima}}
  {\pgfpoint{.25\@tempdima}{.5\@tempdima}}
  {\pgfpoint{-.5\@tempdima}{\@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{)}{(}{(}{)}




% A pointed bracket shaped arrow

\pgfarrowsdeclare{angle 90}{angle 90}
{
  \@tempdima=0.3pt%
  \advance\@tempdima by.25\pgflinewidth%
  \@tempdimb=5.5\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=.5\@tempdima\advance\@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.3pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpoint{-5.5\@tempdima}{-6\@tempdima}}
  \pgfpathlineto{\pgfpoint{0.5\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{-5.5\@tempdima}{6\@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{angle 90 reversed}{angle 90 reversed}{angle 90}{angle 90}


\pgfarrowsdeclare{angle 60}{angle 60}
{
  \@tempdima=0.3pt%
  \advance\@tempdima by.25\pgflinewidth%
  \@tempdimb=7.29\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=.5\@tempdima\advance\@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.3pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{150}{9\@tempdima}}}
  \pgfpathlineto{\pgfpoint{0.5\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{-150}{9\@tempdima}}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{angle 60 reversed}{angle 60 reversed}{angle 60}{angle 60}



\pgfarrowsdeclare{angle 45}{angle 45}
{
  \@tempdima=0.3pt%
  \advance\@tempdima by.25\pgflinewidth%
  \@tempdimb=8.705\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=.5\@tempdima\advance\@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.3pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{157}{10\@tempdima}}}
  \pgfpathlineto{\pgfpoint{0.5\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{-157}{10\@tempdima}}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{angle 45 reversed}{angle 45 reversed}{angle 45}{angle 45}



% A dot shaped arrow

\pgfarrowsdeclare{*}{*}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \@tempdimb=5.5\@tempdima\advance\@tempdimb by\pgflinewidth
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=1.5\@tempdima\advance\@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfpathcircle{\pgfpoint{-3\@tempdima}{0pt}}{4.5\@tempdima}
  \pgfusepathqfillstroke
}


% An open dot shaped arrow

\pgfarrowsdeclare{o}{o}
{
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \@tempdimb=9\@tempdima\advance\@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfpathcircle{\pgfpoint{4.5\@tempdima}{0bp}}{4.5\@tempdima}
  \pgfusepathqstroke
}



% A diamond shaped arrow

\pgfarrowsdeclare{diamond}{diamond}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.275\pgflinewidth%
  \@tempdimb=13\@tempdima\advance\@tempdimb by.5\pgflinewidth
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=1\@tempdima\advance\@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.275\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{1\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{-6\@tempdima}{4\@tempdima}}
  \pgfpathlineto{\pgfpoint{-13\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{-6\@tempdima}{-4\@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclare{open diamond}{open diamond}%{{-.5bp}{14.5bp}}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.275\pgflinewidth%
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdimb=14\@tempdima\advance\@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.275\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{14\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{7\@tempdima}{4\@tempdima}}
  \pgfpathlineto{\pgfpoint{0\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{7\@tempdima}{-4\@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



% A triangle shaped arrow

\pgfarrowsdeclare{triangle 90}{triangle 90}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \@tempdimb=5.5\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=.5\@tempdima\advance\@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpoint{-5.5\@tempdima}{-6\@tempdima}}
  \pgfpathlineto{\pgfpoint{0.5\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{-5.5\@tempdima}{6\@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{triangle 90 reversed}{triangle 90 reversed}{triangle 90}{triangle 90}


\pgfarrowsdeclare{triangle 60}{triangle 60}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \@tempdimb=7.29\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=.5\@tempdima\advance\@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{150}{9\@tempdima}}}
  \pgfpathlineto{\pgfpoint{0.5\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{-150}{9\@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{triangle 60 reversed}{triangle 60 reversed}{triangle 60}{triangle 60}




\pgfarrowsdeclare{triangle 45}{triangle 45}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \@tempdimb=8.705\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=.5\@tempdima\advance\@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{157}{10\@tempdima}}}
  \pgfpathlineto{\pgfpoint{0.5\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfpoint{0.5\@tempdima}{0pt}}{\pgfpointpolar{-157}{10\@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{triangle 45 reversed}{triangle 45 reversed}{triangle 45}{triangle 45}




\pgfarrowsdeclare{open triangle 90}{open triangle 90}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdimb=6\@tempdima\advance\@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpoint{0\@tempdima}{-6\@tempdima}}
  \pgfpathlineto{\pgfpoint{6\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{0\@tempdima}{6\@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}

\pgfarrowsdeclare{open triangle 90 reversed}{open triangle 90 reversed}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{-.707\pgflinewidth}
  \@tempdimb=6\@tempdima\advance\@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpoint{6\@tempdima}{-6\@tempdima}}
  \pgfpathlineto{\pgfpoint{0\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{6\@tempdima}{6\@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 60}{open triangle 60}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdimb=7.794\@tempdima\advance\@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfpoint{7.794\@tempdima}{0pt}}{\pgfpointpolar{150}{9\@tempdima}}}
  \pgfpathlineto{\pgfpoint{7.794\@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfpoint{7.794\@tempdima}{0pt}}{\pgfpointpolar{-150}{9\@tempdima}}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 60 reversed}{open triangle 60 reversed}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{-\pgflinewidth}
  \@tempdimb=7.794\@tempdima\advance\@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointpolar{30}{9\@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfpointpolar{-30}{9\@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 45}{open triangle 45}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdimb=9.205\@tempdima\advance\@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfpoint{9.205\@tempdima}{0pt}}{\pgfpointpolar{157}{10\@tempdima}}}
  \pgfpathlineto{\pgfpoint{9.205\@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfpoint{9.205\@tempdima}{0pt}}{\pgfpointpolar{-157}{10\@tempdima}}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 45 reversed}{open triangle 45 reversed}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{-1.28\pgflinewidth}
  \@tempdimb=9.205\@tempdima\advance\@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.5pt%
  \advance\@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointpolar{23}{10\@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfpointpolar{-23}{10\@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



% A less fleshy variant of LaTeX's orginal arrow type

\pgfarrowsdeclare{latex'}{latex'}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{-4\@tempdima}
  \pgfarrowsrightextend{6\@tempdima}
}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfpoint{6\@tempdima}{0\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{3.5\@tempdima}{.5\@tempdima}}
  {\pgfpoint{-1\@tempdima}{1.5\@tempdima}}
  {\pgfpoint{-4\@tempdima}{3.75\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-1.5\@tempdima}{1\@tempdima}}
  {\pgfpoint{-1.5\@tempdima}{-1\@tempdima}}
  {\pgfpoint{-4\@tempdima}{-3.75\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-1\@tempdima}{-1.5\@tempdima}}
  {\pgfpoint{3.5\@tempdima}{-.5\@tempdima}}
  {\pgfpoint{6\@tempdima}{0\@tempdima}}
  \pgfusepathqfill
}

\pgfarrowsdeclarereversed{latex' reversed}{latex' reversed}{latex'}{latex'}


% A rounded variant of the stealth arrow

\pgfarrowsdeclare{stealth'}{stealth'}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \@tempdimb=6\@tempdima\advance\@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{-\@tempdimb}
  \@tempdimb=2\@tempdima\advance\@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{2\@tempdima}{0\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-.5\@tempdima}{.5\@tempdima}}
  {\pgfpoint{-3\@tempdima}{1.5\@tempdima}}
  {\pgfpoint{-6\@tempdima}{3.25\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-3\@tempdima}{1\@tempdima}}
  {\pgfpoint{-3\@tempdima}{-1\@tempdima}}
  {\pgfpoint{-6\@tempdima}{-3.25\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-3\@tempdima}{-1.5\@tempdima}}
  {\pgfpoint{-.5\@tempdima}{-.5\@tempdima}}
  {\pgfpoint{2\@tempdima}{0\@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{stealth' reversed}{stealth' reversed}{stealth'}{stealth'}



% The two half of the $\to$ arrow

\pgfarrowsdeclare{left to}{left to}
{
  \@tempdima=-0.84pt%
  \advance\@tempdima by-1.3\pgflinewidth%
  \@tempdimb=0.21pt%
  \advance\@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{\@tempdima}
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-3\@tempdima}{4\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-2.75\@tempdima}{2.5\@tempdima}}
  {\pgfpoint{0pt}{0.25\@tempdima}}
  {\pgfpoint{0.75\@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfpoint{0.55\@tempdima}{-0.125\pgflinewidth}}
  {\pgfpoint{0.5\@tempdima}{-0.125\pgflinewidth}}
  {\pgfpoint{0.5\@tempdima}{-0.125\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{0pt}{-0.125\pgflinewidth}}
  \pgfusepathqstroke
}


\pgfarrowsdeclare{right to}{right to}
{
  \@tempdima=-0.84pt%
  \advance\@tempdima by-1.3\pgflinewidth%
  \@tempdimb=0.21pt%
  \advance\@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{\@tempdima}
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-3\@tempdima}{-4\@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-2.75\@tempdima}{-2.5\@tempdima}}
  {\pgfpoint{0pt}{-0.25\@tempdima}}
  {\pgfpoint{0.75\@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfpoint{0.55\@tempdima}{0.125\pgflinewidth}}
  {\pgfpoint{0.5\@tempdima}{0.125\pgflinewidth}}
  {\pgfpoint{0.5\@tempdima}{0.125\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{0pt}{0.125\pgflinewidth}}
  \pgfusepathqstroke
}



% The halfs of the $\to$ arrow reversed

\pgfarrowsdeclare{left to reversed}{left to reversed}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{-.1\pgflinewidth}
  \@tempdimb=3.75\@tempdima\advance\@tempdimb by0.9\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfpoint{3.75\@tempdima}{4\@tempdima}}
    \pgfpathcurveto{\pgfpoint{3.5\@tempdima}{2.5\@tempdima}}{\pgfpoint{0.75\@tempdima}{0.25\@tempdima}}{\pgfpoint{0pt}{0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfpoint{3.75\@tempdima}{4\@tempdima}}
    \pgfpathcurveto{\pgfpoint{3.5\@tempdima}{2.5\@tempdima}}{\pgfpoint{0.75\@tempdima}{0.25\@tempdima}}{\pgfpoint{0pt}{-0.125\pgflinewidth}}
  }
  \pgfusepathqstroke%
}

\pgfarrowsdeclare{right to reversed}{right to reversed}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{-.1\pgflinewidth}
  \@tempdimb=3.75\@tempdima\advance\@tempdimb by0.9\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.28pt%
  \advance\@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfpoint{3.75\@tempdima}{-4\@tempdima}}
    \pgfpathcurveto{\pgfpoint{3.5\@tempdima}{-2.5\@tempdima}}{\pgfpoint{0.75\@tempdima}{-0.25\@tempdima}}{\pgfpoint{0pt}{-0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfpoint{3.75\@tempdima}{-4\@tempdima}}
    \pgfpathcurveto{\pgfpoint{3.5\@tempdima}{-2.5\@tempdima}}{\pgfpoint{0.75\@tempdima}{-0.25\@tempdima}}{\pgfpoint{0pt}{0.125\pgflinewidth}}
  }
  \pgfusepathqstroke%
}



% A left hook

\pgfarrowsdeclare{left hook}{left hook}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdimb=3.75\@tempdima\advance\@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpoint{0\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{0.75\@tempdima}{0\@tempdima}}
  \pgfpathcurveto{\pgfpoint{2.415\@tempdima}{0\@tempdima}}{\pgfpoint{3.75\@tempdima}{1.665\@tempdima}}{\pgfpoint{3.75\@tempdima}{3\@tempdima}}
  \pgfpathcurveto{\pgfpoint{3.75\@tempdima}{4.665\@tempdima}}{\pgfpoint{2.415\@tempdima}{6\@tempdima}}{\pgfpoint{0.75\@tempdima}{6\@tempdima}}
  \pgfusepathqstroke%
}

\pgfarrowsdeclarereversed{left hook reversed}{left hook reversed}{left hook}{left hook}



% A right hook

\pgfarrowsdeclare{right hook}{right hook}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdimb=3.75\@tempdima\advance\@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpoint{0\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{0.75\@tempdima}{0\@tempdima}}
  \pgfpathcurveto{\pgfpoint{2.415\@tempdima}{0\@tempdima}}{\pgfpoint{3.75\@tempdima}{-1.665\@tempdima}}{\pgfpoint{3.75\@tempdima}{-3\@tempdima}}
  \pgfpathcurveto{\pgfpoint{3.75\@tempdima}{-4.665\@tempdima}}{\pgfpoint{2.415\@tempdima}{-6\@tempdima}}{\pgfpoint{0.75\@tempdima}{-6\@tempdima}}
  \pgfusepathqstroke%
}

\pgfarrowsdeclarereversed{right hook reversed}{right hook reversed}{right hook}{right hook}


% Hooks in both directions

\pgfarrowsdeclare{hooks}{hooks}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{-.5\pgflinewidth}
  \@tempdimb=3.75\@tempdima\advance\@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{\@tempdimb}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpoint{0\@tempdima}{0\@tempdima}}
  \pgfpathlineto{\pgfpoint{0.75\@tempdima}{0\@tempdima}}
  \pgfpathcurveto{\pgfpoint{2.415\@tempdima}{0\@tempdima}}{\pgfpoint{3.75\@tempdima}{1.665\@tempdima}}{\pgfpoint{3.75\@tempdima}{3\@tempdima}}
  \pgfpathcurveto{\pgfpoint{3.75\@tempdima}{4.665\@tempdima}}{\pgfpoint{2.415\@tempdima}{6\@tempdima}}{\pgfpoint{0.75\@tempdima}{6\@tempdima}}
  \pgfpathmoveto{\pgfpoint{0.75\@tempdima}{0\@tempdima}}
  \pgfpathcurveto{\pgfpoint{2.415\@tempdima}{0\@tempdima}}{\pgfpoint{3.75\@tempdima}{-1.665\@tempdima}}{\pgfpoint{3.75\@tempdima}{-3\@tempdima}}
  \pgfpathcurveto{\pgfpoint{3.75\@tempdima}{-4.665\@tempdima}}{\pgfpoint{2.415\@tempdima}{-6\@tempdima}}{\pgfpoint{0.75\@tempdima}{-6\@tempdima}}
  \pgfusepathqstroke%
}

\pgfarrowsdeclarereversed{hooks reversed}{hooks reversed}{hooks}{hooks}


% An arrow that looks like a serif of the computer modern font

\pgfarrowsdeclare{serif cm}{serif cm}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.45\pgflinewidth%
  \pgfarrowsleftextend{-.75\@tempdima}
  \pgfarrowsrightextend{.04\pgflinewidth}
}
{
  \@tempdima=0.4pt%
  \advance\@tempdima by.45\pgflinewidth%
  \pgftransformxshift{.04\pgflinewidth}
  \pgfpathmoveto{\pgfpoint{-.75\@tempdima}{.5\pgflinewidth}}
  \pgfpathcurveto
    {\pgfpoint{-.375\@tempdima}{.5\pgflinewidth}}
    {\pgfpoint{-.375\@tempdima}{.7\pgflinewidth}}
    {\pgfpoint{-.375\@tempdima}{1.95\@tempdima}}
  \pgfpathlineto{\pgfpoint{0pt}{1.95\@tempdima}}
  \pgfpathcurveto
    {\pgfpoint{-.04\pgflinewidth}{.5\@tempdima}}
    {\pgfpoint{-.04\pgflinewidth}{-.5\@tempdima}}
    {\pgfpoint{0pt}{-1.95\@tempdima}}  
  \pgfpathlineto{\pgfpoint{-.375\@tempdima}{-1.95\@tempdima}}  
  \pgfpathcurveto
    {\pgfpoint{-.375\@tempdima}{-.7\pgflinewidth}}
    {\pgfpoint{-.375\@tempdima}{-.5\pgflinewidth}}
    {\pgfpoint{-.75\@tempdima}{-.5\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}



% Round cap

\pgfarrowsdeclare{round cap}{round cap}
{\pgfarrowsleftextend{0pt}\pgfarrowsrightextend{\pgflinewidth}}
{
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}


% Butt cap

\pgfarrowsdeclare{butt cap}{butt cap}
{\pgfarrowsleftextend{-.1\pgflinewidth}\pgfarrowsrightextend{.5\pgflinewidth}}
{
  \pgfsetdash{}{0pt}
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfpoint{-.1\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}



% 90 degrees cap

\pgfarrowsdeclare{triangle 90 cap}{triangle 90 cap}
{\pgfarrowsleftextend{-.1\pgflinewidth}\pgfarrowsrightextend{1\pgflinewidth}}
{
  \pgfpathmoveto{\pgfpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfusepathqfill
}


% reversed 90 degrees cap

\pgfarrowsdeclare{triangle 90 cap reversed}{triangle 90 cap reversed}
{\pgfarrowsleftextend{-.1\pgflinewidth}\pgfarrowsrightextend{1\pgflinewidth}}
{
  \pgfpathmoveto{\pgfpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{-.1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{-.1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{0.5\pgflinewidth}{0\pgflinewidth}}
  \pgfusepathqfill
}



% fast

\pgfarrowsdeclare{fast cap}{fast cap}
{\pgfarrowsleftextend{-.1\pgflinewidth}\pgfarrowsrightextend{2\pgflinewidth}}
{
  \pgfpathmoveto{\pgfpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{2\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}


\pgfarrowsdeclare{fast cap reversed}{fast cap reversed}
{\pgfarrowsleftextend{-.1\pgflinewidth}\pgfarrowsrightextend{2\pgflinewidth}}
{
  \pgfpathmoveto{\pgfpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{2\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{2\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1.5\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}


\endinput


==> pgflibrarypatterns.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarypatterns.code.tex,v 1.7 2006/10/11 15:22:26 tantau Exp $


% Lines in different directions

\pgfdeclarepatternformonly{horizontal lines}{\pgfpointorigin}{\pgfpoint{100pt}{1pt}}{\pgfpoint{100pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfpoint{0pt}{0.5pt}}
  \pgfpathlineto{\pgfpoint{100pt}{0.5pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{vertical lines}{\pgfpointorigin}{\pgfpoint{1pt}{100pt}}{\pgfpoint{3pt}{100pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfpoint{0.5pt}{0pt}}
  \pgfpathlineto{\pgfpoint{0.5pt}{100pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{north east lines}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{4pt}{4pt}}{\pgfpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfpoint{3.1pt}{3.1pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{north west lines}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{4pt}{4pt}}{\pgfpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfpoint{0pt}{3pt}}
  \pgfpathlineto{\pgfpoint{3.1pt}{-0.1pt}}
  \pgfusepath{stroke}
}

% Crossed lines in different directions

\pgfdeclarepatternformonly{grid}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{4pt}{4pt}}{\pgfpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfpoint{0pt}{3.1pt}}
  \pgfpathmoveto{\pgfpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfpoint{3.1pt}{0pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{crosshatch}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{4pt}{4pt}}{\pgfpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfpoint{3.1pt}{0pt}}
  \pgfpathlineto{\pgfpoint{0pt}{3.1pt}}
  \pgfpathmoveto{\pgfpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfpoint{3.1pt}{3.1pt}}
  \pgfusepath{stroke}
}


% Dotted regions

\pgfdeclarepatternformonly{dots}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{1pt}{1pt}}{\pgfpoint{3pt}{3pt}}%
{
  \pgfpathcircle{\pgfpoint{0pt}{0pt}}{.5pt}
  \pgfusepath{fill}
}

\pgfdeclarepatternformonly{crosshatch dots}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{2.5pt}{2.5pt}}{\pgfpoint{3pt}{3pt}}%
{
  \pgfpathcircle{\pgfpoint{0pt}{0pt}}{.5pt}
  \pgfpathcircle{\pgfpoint{1.5pt}{1.5pt}}{.5pt}
  \pgfusepath{fill}
}




% Star shaped patterns

\pgfdeclarepatternformonly{fivepointed stars}{\pgfpointorigin}{\pgfpoint{3mm}{3mm}}{\pgfpoint{3mm}{3mm}}%
{
  \pgftransformshift{\pgfpoint{1mm}{1mm}}
  \pgfpathmoveto{\pgfpointpolar{18}{1mm}}
  \pgfpathlineto{\pgfpointpolar{162}{1mm}}
  \pgfpathlineto{\pgfpointpolar{306}{1mm}}
  \pgfpathlineto{\pgfpointpolar{90}{1mm}}
  \pgfpathlineto{\pgfpointpolar{234}{1mm}}
  \pgfpathclose%
  \pgfusepath{fill}
}

\pgfdeclarepatternformonly{sixpointed stars}{\pgfpointorigin}{\pgfpoint{3mm}{3mm}}{\pgfpoint{3mm}{3mm}}%
{
  \pgftransformshift{\pgfpoint{1mm}{1mm}}
  \pgfpathmoveto{\pgfpointpolar{30}{1mm}}
  \pgfpathlineto{\pgfpointpolar{150}{1mm}}
  \pgfpathlineto{\pgfpointpolar{270}{1mm}}
  \pgfpathclose%
  \pgfpathmoveto{\pgfpointpolar{-30}{1mm}}
  \pgfpathlineto{\pgfpointpolar{-270}{1mm}}
  \pgfpathlineto{\pgfpointpolar{-150}{1mm}}
  \pgfpathclose%
  \pgfsetnonzerorule
  \pgfusepath{fill}
}



% Bricks

\pgfdeclarepatternformonly{bricks}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{5mm}{5mm}}{\pgfpoint{4mm}{4mm}}%
{
  \pgfsetlinewidth{0.8pt}
  \pgfpathmoveto{\pgfpoint{0mm}{1mm}}
  \pgfpathlineto{\pgfpoint{4mm}{1mm}}
  \pgfpathmoveto{\pgfpoint{0mm}{3mm}}
  \pgfpathlineto{\pgfpoint{4mm}{3mm}}
  \pgfpathmoveto{\pgfpoint{1mm}{0mm}}
  \pgfpathlineto{\pgfpoint{1mm}{1mm}}
  \pgfpathmoveto{\pgfpoint{3mm}{1mm}}
  \pgfpathlineto{\pgfpoint{3mm}{3mm}}
  \pgfpathmoveto{\pgfpoint{1mm}{3mm}}
  \pgfpathlineto{\pgfpoint{1mm}{4mm}}
  \pgfusepath{stroke}
}




\endinput


==> pgflibrarytikzarrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzarrows.code.tex,v 1.2 2006/10/11 15:22:26 tantau Exp $

\usepgflibrary{arrows}

\endinput


==> pgflibrarytikzer.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzer.code.tex,v 1.3 2006/10/11 15:22:26 tantau Exp $


% Styles for entity types:

\tikzstyle{every entity}=           []
\tikzstyle{entity}=                 [rectangle,draw,
                                     minimum height=2\baselineskip,
                                     minimum width=4\baselineskip,every entity]


% Styles for relationship types:

\tikzstyle{every relationship}=     []
\tikzstyle{relationship}=           [diamond,draw,
                                     minimum size=1.5\baselineskip,
                                     inner sep=1pt,
                                     every relationship]


% Styles for relationship types:

\tikzstyle{every attribute}=        []
\tikzstyle{attribute}=              [minimum size=1.5\baselineskip,ellipse,draw,every attribute]
\tikzstyle{key attribute}=          [font=\itshape,attribute]




\endinput


==> pgflibrarytikzpatterns.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzpatterns.code.tex,v 1.2 2006/10/11 15:22:26 tantau Exp $

\usepgflibrary{patterns}

\endinput


==> pgflibrarytikzplothandlers.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzplothandlers.code.tex,v 1.2 2006/10/11 15:22:26 tantau Exp $

\usepgflibrary{plothandlers}

\endinput


==> pgflibrarytikzplotmarks.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzplotmarks.code.tex,v 1.2 2006/10/11 15:22:26 tantau Exp $

\usepgflibrary{plotmarks}

\endinput


==> pgflibrarytikzshapes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzshapes.code.tex,v 1.2 2006/10/11 15:22:26 tantau Exp $

\usepgflibrary{shapes}

\endinput


==> pgflibrarytikzsnakes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzsnakes.code.tex,v 1.2 2006/10/11 15:22:26 tantau Exp $

\usepgflibrary{snakes}

\endinput

